GreedyML: A Parallel Algorithm for Maximizing Constrained Submodular Functions

We describe a parallel approximation algorithm for maximizing monotone submodular functions subject to hereditary constraints on distributed memory multiprocessors. Our work is motivated by the need to solve submodular optimization problems on massive data sets, for practical contexts such as data summarization, machine learning, and graph sparsification. Our work builds on the randomized distributed RandGreedi algorithm, proposed by Barbosa, Ene, Nguyen, and Ward (2015). This algorithm computes a distributed solution by randomly partitioning the data among all the processors and then employing \emph{a single} accumulation step in which all processors send their partial solutions to one processor. However, for large problems, the accumulation step exceeds the memory available on a processor, and the processor that performs the accumulation becomes a computational bottleneck. Hence we propose a generalization of the RandGreedi algorithm that employs multiple accumulation steps to reduce the memory required. We analyze the approximation ratio and the time complexity of the algorithm (in the BSP model). We evaluate the new GreedyML algorithm on three classes of problems, and report results from large-scale data sets with millions of elements. The results show that the GreedyML algorithm can solve problems where the sequential Greedy and distributed RandGreedi algorithms fail due to memory constraints. For certain computationally intensive problems, the GreedyML algorithm is faster than the RandGreedi algorithm. The observed approximation quality of the solutions computed by the GreedyML algorithm closely matches those obtained by the RandGreedi algorithm on these problems.

==> Latest/algAnalysis.tex <==
\section{Analysis of Our Algorithm} 
In this section, we will derive the expected approximation ratio of the \greedyl{} algorithm. We will then describe the three submodular functions we experiment with and derive their computation and communication complexities.


\subsection{Expected Approximation Ratio} 

This subsection proves the expected approximation ratio of our \greedyl\ algorithm in Theorem~\ref{thm:approx}. To do so, we need 
three  Lemmas.
The first Lemma characterizes elements that do not change the 
solution computed by the \greedyl algorithm. 
We need some preliminary notation. 
When we wish to indicate the data set that a node in the tree and its descendants work with, we add an argument to $\greedyl(\ell, id)$, and write  $\greedyl(V_{\ell, id}, \ell, id)$.
When we perform a union operation on this data set with some set $B$, and execute the \greedyl\ algorithm on the union, i.e.,  $\greedyl(V_{\ell, id}\cup B, \ell, id)$,  
then elements in $B$ are assigned randomly to the leaves of the subtree rooted at node $(\ell, id)$ and the algorithm is run with the updated data sets. 
Lemma \ref{lem:stable} compares executions of the algorithm when this union operation is performed for a special set $B$. It states that if adding an individual element of a set, $B$, to the input of the \greedyl{} does not change the solution set then adding the whole set, $B$ to the input will also have no effect on the solution. Here we consider executions that use the same random tape, number of machines, and branching factor. 
We use the same random tape to couple the executions. Therefore, the result of the Lemma is not over the expectation of the random tape.
\begin{lemma}
\label{lem:stable}
Let $T(m, L, b)$ be an accumulation tree. 
 Consider a universal set $W$, and a random tape $r_W$
 that maps elements of $W$ to the leaves of $T$.
 Let $V \subseteq W$ denote the set of elements accessible to 
 a node $(\ell, id)$, and consider adding elements of $B \subseteq W$ to this node. 
If we have \greedyl$(V \cup \{e\} , \ell,id) = \greedyl(V, \ell,id) $, for each element $e\in B$, then $\greedyl(V \cup B, \ell,id) = \greedyl(V, \ell,id)$.
\end{lemma} 


Note: Function calls in this analysis use the same random tape for assigning elements; hence elements are assigned uniformly at random to the machines, but they use the same random assignment in all runs involving $V$;  $V \cup \{e\}, \forall e\in B$;  \text{ and } $V\cup B$.
\begin{proof}
 If possible, let $\greedyl(V \cup B, \ell,id) \neq \greedyl(V, \ell,id)$. Let $e$ be the first element of $B$ to be selected by the \greedy\ algorithm at the final level. 
 Let $i$ be the level in which $e$ was in the input in some machine but not selected in a solution for the next level in $\greedyl(V \cup \{ e\}, \ell, id)$. 
 Since $e$ is the first element of $B$ that was selected by the \greedy\ algorithm, the elements chosen before it at level $i$ in $\greedyl(V \cup B, \ell, id)$ are the same ones chosen before it at level $i$ in $\greedyl(V \cup \{e\}, \ell, id)$. Since it was not selected in $\greedyl(V \cup \{e\}, \ell, id)$ it will not be selected in $\greedyl(V \cup B, \ell, id)$. 
 This is a contradiction since $e$ must be selected at every level to be present in the final solution.
\end{proof}

Now we turn to the two Lemmas that 
provide bounds on the quality of the computed solutions in terms of the optimal solution at an internal node in the accumulation tree. 

Lemma~\ref{lem:individual} provides a lower bound on the expected function value of the solution of the  \greedyl\ algorithm from a child of the internal node. 
Lemma~\ref{lem:accumulate} provides a lower bound on the expected function value of the solution set from the \greedy\ algorithm executed at each internal node on the union of the partial solutions from its children. 
These Lemmas depend on the probability distribution defined below.

Let $p_{\ell, id}\colon V_{\ell, id}  \to [0,1]$ be a probability distribution over the elements in $V_{\ell, id}$, which we shall define below.  
Here $ A \sim V_{\ell, id}(1/b)$ denotes a random subset of $V_{\ell, id}$ such that each element is independently present in $A$ with probability $1/b$.
This probability corresponds to the distribution from the random tape because each element is present with the same likelihood from any child of the node. Let $OPT_{\ell, id}$ be an optimal solution of the constrained submodular maximization problem when the input data is $V_{\ell, id}$.

The probability $p_{\ell,id}$ is defined as follows:  
\begin{equation*}
    p_{\ell,id}(e) = 
    \begin{cases} 
    \Pr\limits_{A \sim V_{\ell, id}(1/b)}
 \left[\greedyl(A\cup \{e\}, \ell-1, id) 
\right],  & \text{if} \  e\in OPT_{\ell,id};\\ 
 0,  & \text{otherwise.} 
\end{cases} 
\end{equation*}
For any internal node $(\ell,id)$, the distribution $p_{\ell,id}$ defines { 
the probability that each  element of $OPT_{\ell,id}$

is in the solution of the \greedyl\ algorithm of a child when it is accessible to the child node.} 

Next, we state and prove Lemma~\ref{lem:individual} that relates the expected solution of the \greedyl\ algorithm at a child node with the optimal solution at the 
node when the approximation ratio of the \greedyl\  algorithm at the child is $\beta$. \color{black}
\begin{lemma}
\label{lem:individual}
Let $c = (\ell-1, id_c)$ be a child of an internal node $n = (\ell,id)$ of the accumulation tree.   Let $S_c$ be the solution computed from child $c$, and $V_c \subset V_{n}$ denote the elements considered in forming $S_c$. If $\mathbb{E}_{V_c}[f(S_c)] \geq \beta \cdot f(OPT_{\ell-1,id_c})$, then 
$$    \mathop{\mathbb{E}}_{V_n}[f(S_c)] \geq \beta \cdot \fhat(1_{OPT_{\ell,id}}-p_{\ell,id}). 
$$
\end{lemma}

\begin{proof}
We first construct a subset of $OPT_{\ell, id}$ that contains all the elements that do not appear in $S_c$ when added to some leaf node in the subtree rooted at child $c$.
Let $O_c$ be the rejected set that can be added to $V_c$ without changing $S_c$; i.e., 
$$O_c =  \{ e \in OPT_{\ell,id} :  e \notin \greedyl(V_c \cup \{e\}, \ell', id )\}.$$
 
To clarify further, $O_c$ is a randomized set dependent on the tape $r_{V_{\ell,id}}$. Since the distribution of $V_c$ is the same as $V_{\ell,id}(1/b)$ for each element $e$ in $OPT_{\ell,id}$, 
\begin{equation}
    \Pr[e \in O_c] = 1 - \Pr[e \notin O_c] = 1- p_{\ell,id}(e). \label{eqn:E[Oc]}
\end{equation}
From Lemma~\ref{lem:stable}, we know that $\greedyl(V_c \cup O_c,\ell-1,id_c ) = \greedyl(V_c,\ell-1,id_c) $ .  
Since the rejected set $O_c \subseteq OPT_{\ell, id}$ and the constraints are hereditary, $O_c \in \mathcal{C}$ (i.e $O_c$ is a feasible solution of child node c).
\begin{equation}
    f(OPT_{\ell-1,id_c}) \geq f(O_c). \label{eqn:OcF}
\end{equation}
Then from the condition of Lemma \ref{lem:individual}, we have
\vspace{-2.5mm}

\begin{align*}
\mathbb{E}_{V_n}[\mathbb{E}_{V_c}f(S_c)] &\geq \beta \cdot \mathbb{E}_{V_n}[f(OPT_{\ell-1,id_c})] \\ 
    % & \text{(condition of Lemma~2)} \notag \\
    \mathbb{E}_{V_n}[f(S_c)] &\geq \beta \cdot \mathbb{E}_{V_n}[f(OPT_{\ell-1,id_c})]  
    & \pushright{[ V_c \subset V_n]}  \notag \\
    &\geq \beta \cdot \fhat(\mathbb{E}_{V_n}[1_{O_c}])
    & \pushright{[\text{Eqn.} (\ref{eqn:OcF})]} \notag \\
    & \geq \beta \cdot \mathbb{E}_{V_n}[f(O_c)]  
    &\pushright{[\text{\lsz~(2)},\ref{eqn:Lova}]}  \notag\\ 
    &\geq \beta \cdot f^-(\mathbb{E}_{V_n}[1_{O_c}])
     = \beta\cdot \fhat(1_{OPT_{\ell,id}} - p_{\ell,id})
    & \pushright{[\text{Eqn.} (\ref{eqn:E[Oc]})].} \notag 
\end{align*}


\end{proof}
Now we show how the solution of the \greedy{} algorithm that runs at each internal node compares with the optimal solution at the internal node.
\begin{lemma}
\label{lem:accumulate}
 For an internal node $n = (\ell, id)$, let $D$ be the union of all the solutions computed by the children of node $n$ in the accumulation tree. Let $S = \greedy(D)$ be the solution from the Greedy algorithm on the set $D$. If \greedy\ is an $\alpha$-approximate algorithm, then    
\newline
{\centerline{$\mathbb{E}_{V_n}[f(S)] \geq \alpha \cdot f^-(p_{\ell, id}).$}} 
\end{lemma}

\begin{proof}
We first show a preliminary result on the union set $D$. Consider an element $e\in D\cap OPT_{\ell, id}$ present in some solution $S_c$ from a child $c$. Then, 
$$\Pr[e\in S_c | e \in V_c]
    = \Pr[e\in \greedyl(V_c,\ell-1,id) | e \in V_c]. $$

Since the distribution of $V_c \sim V_{\ell,id}(1/b)$ conditioned on $e \in V_c$ is identical to the distribution of $B \cup \{e\}$, where $B \sim V_{\ell,id}(1/b)$,  we have,
$$
\Pr[e\in S_c | e \in V_c] = \Pr_{B \sim V_{\ell, id}(1/b)}[ e \in \greedyl(B \cup \{e\}, \ell-1,id)]  = p_{\ell,id}(e).
$$
  
Since this result holds for every child $c$, and each subset $V_c$  is disjoint from the corresponding subsets mapped to the other children,  we have 
\begin{equation}
    \Pr(D\cap OPT_{\ell,id}) = p_{\ell,id}. \label{eqn:PrD}
\end{equation} 
 Now, we are ready to prove the Lemma. 
 The subset $D \cap OPT_{\ell, id} \in \mathcal{C}$, since it is a subset of $OPT_{\ell, id}$ and the constraints are hereditary. Further, since the \greedy\ algorithm is $\alpha$-approximate, we have 
\begin{align}
    f(S) &\geq \alpha \cdot f(D\cap OPT_{\ell,id}) \notag \\
\mathbb{E}_{V_n}[f(S)] &\geq \mathbb{E}_{V_n}[\alpha\cdot f(D\cap OPT_{\ell,id})] \notag \\
    &\geq \alpha\cdot \mathbb{E}_{V_n}[f(D\cap OPT_{\ell,id})] \notag \\
    &\geq \alpha\cdot \fhat(\mathbb{E}_{V_n}[1_{D\cap OPT_{\ell,id}}]) 
    & \pushright{[\text{\lsz Ext.~(2)}, \ref{eqn:Lova}}]  %\ref{eqn:Lov2}})}
    \notag \\
    & = \alpha\cdot \fhat(p_{\ell,id}).  
    & \pushright{[\text{Eqn.}\ref{eqn:PrD}].}  \label{eqn:lemma3} 
\end{align} 
\end{proof}

\begin{theorem}
\label{thm:approx}
Let $T(m, L,b)$ be an accumulation tree.  
For a universal set $W$ and random tape $r_W$ that maps elements of $W$ to the leaves of the tree $T$,  let $V_{\ell, id} \subseteq W$ denote the subset of $W$ accessible to a node $(\ell, id)$. 
Let $OPT_{\ell, id}$ be an optimal solution computed from the subset $V_{\ell, id}$ for the submodular function $f$ with constraints $\mathcal{C}$.  
If \greedy\ is an $\alpha$-approximate algorithm,  then 
$$
{ \mathbb{E}_{V_{\ell,id}}\left[f(\greedyl(V_{\ell,id}, \ell,id))\right] \geq \dfrac{\alpha}{(\ell+1)} f(OPT_{\ell,id}).}
$$
\end{theorem}


\begin{proof}
 We prove this theorem by induction on the level $\ell$.

\textbf{Base case}, $\ell=0$: Here, there is no accumulation step,
and we obtain the solution from a single node. Thus we run the \greedy\ algorithm on $V_{\ell, id}$. The result follows since the \greedy\ algorithm has the approximation ratio $\alpha$. 

\textbf{Inductive case}, $\ell = \ell' + 1$: 
We first obtain a relation for the quality of the solutions at level $\ell'$ compared to the quality of an optimal solution. 

For each child c, let $S_c$ be a solution computed by the 
\greedyl\ algorithm from the data  $V_c \subset V_{\ell, id}$; 

From the \textbf{induction hypothesis} applied to child $c=(\ell',id)$,  the approximation ratio obtained as a result of the computation $\greedyl(V_c,\ell',id )$ is $\alpha/(\ell'+ 1) = \alpha/\ell$. This  implies that $\mathbb{E}_{V_{l',id}}[f(S_c)] \geq \frac{\alpha}{\ell}\cdot f^-(1_{OPT_{\ell',id}}).$ Therefore we can apply Lemma~\ref{lem:individual} to get 
\begin{equation}
    \mathbb{E}_{V_{\ell,id}}[f(S_c)] \geq \frac{\alpha}{\ell}\cdot \fhat(1_{OPT_{\ell,id}}- p_{\ell,id}). \label{eqn:EfSc}
\end{equation}  

After obtaining the solutions from the children, we get the solution $S$ computed by the \greedy\ algorithm on the union of these solution sets.  
From Lemma~\ref{lem:accumulate}, we have
\begin{equation}
    \mathbb{E}_{V_{\ell,id}}[f(S)] \geq \alpha \cdot \fhat(p_{\ell,id}). \label{eqn:EfS}
\end{equation} 
Now we obtain the relation between the solution at level $\ell'+1$ and the optimal solution. Let the solution set at level $\ell'+1$ be $T$. We have  $T = \arg \max \{f(S), f(S_{c})\}$. Then, we can use the lower bounds calculated earlier in Eqn. \ref{eqn:EfSc} and Eqn. \ref{eqn:EfS} to find lower bounds for $T$. 
\[
    \mathbb{E}_{V_{\ell,id}}[f(T)] \geq \alpha\cdot \fhat(p_{\ell,id})  \text{ and } \mathbb{E}_{V_{\ell,id}}[f(T)] 
    \geq \frac{\alpha}{\ell}\cdot \fhat(1_{OPT_{\ell,id}} - p_{\ell,id}). 
\]
By multiplying the second inequality  by $\ell$ and then adding it to the first, we get
\begin{align*}
   (\ell + 1 )\mathbb{E}_{V_{\ell,id}}[f(T)]& \geq \alpha\cdot ( \fhat(1_{OPT_{\ell,id}} - p_{\ell,id}) + \fhat(p_{\ell,id})) \notag  \\
    & = \alpha\cdot \fhat(1_{OPT_{\ell,id}}). 
    & \pushright{[\text{\lsz Ext.~(2)}, {\ref{eqn:Lova}}]}
    \notag
\end{align*}
Dividing by  by $\ell+1$,  and substituting from \lsz Ext.~(1), \ref{eqn:Lova} we conclude that the algorithm is $\alpha/ (\ell+1) $-approximate.
\end{proof}


\subsection{Submodular Functions and Complexity} 
\label{subsec:complexity} 

Here, we describe three submodular functions that we consider in our experiments and then discuss their computational and communication complexities. 

Our algorithm can handle any hereditary constraint, but in our experiments, we consider only cardinality constraints to keep the computations simple. (More general constraints involve additional computations  to check if an element can be added to the current solution set and satisfy the constraints.)
Cardinality constraints are widely used in various applications such as sensor placement~\cite{krause2008efficient}, text, image, and document summarization~\cite{lin2010multi,lin2011class}, and information gathering~\cite{krause2007near}. The problem of maximizing a submodular function under cardinality constraints can be expressed as follows.
\begin{maxi*}
{S \subseteq V}{f(S)}{} {}
\addConstraint{|S|}{\leq k}.
\end{maxi*}
Here $V$ is the ground set, $f$ is a non-negative monotone submodular function, and $k$ is the size of the solution set $S$. 

In our experiments, We have considered the following three submodular functions.
\subsubsection*{$k$-cover}
\label{func:k-cover}
The first problem we consider is the {\em $k$-cover}. 
Given a ground set B, a collection of subsets $V \subseteq 2^B$,  and an integer $k$, the goal is to select a set $S \subseteq V$ containing $k$ of these subsets to maximize $f(S)= |\bigcup_{S_i \in S}S_i |$. 
 
\subsubsection*{$k$-dominating set}
\label{func:k-dom}  The {\em $k$-dominating set} problem is a special case of the $k$-cover problem defined on graphs with the ground set $V$ as the set of vertices.  
We say a vertex $u \in V$ \emph{dominates} all its adjacent vertices (denoted by $\delta(u)$). Our goal is to select a set $S$ of $k$ vertices to dominate as many vertices as possible, i.e., $f(S) = |\bigcup_{u \in S} \delta(u) |$. The marginal gain of any vertex is the number of vertices in its neighborhood that are not yet dominated. Therefore the problem shows diminishing marginal gains and is submodular. 
%in this graph context.  

\subsubsection*{$k$-medoid problem}
\label{func:k-med}
%\smf{k-medoid needs to be motivated from exemplar-based clustering. See discussion in~\cite{Mirzasoleiman}. SG: Let me know if more is needed }
The {\em $k$-medoid problem}~\cite{k-medoid} is  %\smf{need references?} 
used to compute exemplar-based clustering, where we want to select a set of exemplars (cluster centers) that are representatives of a large dataset. Given a collection of elements in a ground set $V$, and a dissimilarity $d(u,v)$, we define a loss function (denoted by $L$) as the average pairwise dissimilarity between the exemplars ($S$) and the elements of the data set, i.e., $L(S)= \dfrac{1}{|V|} \sum_{u\in V} \min_{v \in S} d(u,v)$. Following~\cite{Mirzasoleiman}, we turn this loss minimization to a submodular maximization problem by setting $f(S)= L(\{e_0\}-L(S \cup \{e_0\}$, where $e_0$ is an auxiliary element specific to the dataset. The goal is to select a subset $S \subseteq V$ of size $k$ representing the exemplars that maximize $f(S)$. 

%Our dataset $V$ consists of images where the dissimilarity between two images is the Euclidean distance between vector representations of the pixels in the images. Here, the auxiliary image $e_0$ is a pixel vector of all zeros. Note that, unlike the other two problems, for the $k$-medoid function, we require access to the full dataset for computing the functional value. Since the dataset is distributed, this poses an issue in the experiment. To overcome this following~\cite{Mirzasoleiman,barbosa}, we calculate the objective function value using only the images available \emph{locally} on each machine. This means the ground set for each machine is just the images present in that machine. The local function value is a good estimate of the global value since the data in each machine is selected uniformly at random\smf{this needs reference. SG: We say that we are following \cite{Mirzasoleiman}}.  

Next, we will analyze the computational and communication complexity of our  \greedyl\ algorithm using the bulk synchronous parallel (BSP) model of parallel computation~\cite{Valiant}.
For the analysis, we will denote the number of elements in the ground set by $n = |V|, $%\smf{V?},
the solution size by $k$, the number of machines by $m$, and the number of levels in the accumulation tree by $L$. 

%\SMF{Can we construct these complexities assuming generic greedy complexity? We can assume g(.) is the number of function calls greedy makes. SG: If g(n) is the number of calls made by greedy for data of size n and selection of size k. Then \randgreedi\ is g(n/m)+ g(mk) and our algorithm is g(n/m) + L*g(bk). I am not sure if this is what you mean. }
\smallskip\noindent\textbf{Computational Complexity.}
The number of objective function calls by the sequential \greedy{} algorithm (shown in Algorithm~\ref{Alg:greedy} is $O(nk)$, since $k$ elements are selected to be in the solution, and we may need to compute $O(n)$ marginal gains for each of them. 
Each machine in \randgreedi{} algorithm makes $O(k(n/m + mk))$ function calls, %\smf{This is not right. The number of function calls should also depend on the number of machines. Do you mean parallel runtime?  SG: I mean parallel run time. I changed the language a little to reflect this. },  
where the second term comes from the accumulation step. Each machine of the \greedyl{} algorithm with branching factor $b$ makes $O(k(n/m + Lbk) )$  calls. Recall that $L = \lceil \log_b{m} \rceil$. 
%\todo{I think, it should be $b=\ceil{m^{1/L}}$}

We note that the time complexity of a function call depends on the specific function being computed.
For example,  in the $k$-coverage and the k-dominating set problems,  computing a function costs $O(\delta)$,  where $\delta$ is the size of the largest itemset for $k$-coverage,  and the maximum degree of a vertex for the vertex dominating set. 
In both cases, the runtime complexity is $O(\delta k(n/m + mk))$ for the \randgreedi,  and $O(\delta k(n/m + Lbk) )$ for the \greedyl\ algorithm.  
%\todo{$lbk \rightarrow Lbk$}
%\SMF{What is the local objective? We did not define it in the k-medoid problem definition section. Also, try avoiding using $\Delta$ for the number of features. SG: Added a statement on local objective. Can you suggest an alternate symbol? $d$?$\delta$?}
The $k$-medoid problem computes a local objective function value and has a complexity of $O(n^\prime \delta)$ where $\delta$ is the number of features, and $n^\prime$ is the number of elements present in the machine. 
For the leaves of the accumulation tree, $n^{\prime} = n/m$, and 
for interior nodes, $n^{\prime} = bk$. 
Therefore its complexity is $O(k \delta ((n/m)^2 + (mk)^2))$ for the \randgreedi{},  and $O(k \delta ((n/m)^2 + L(bk)^2) )$ for the \greedyl{} algorithm. %\smf{no $n^\prime$ in the complexity?}  

\smallskip\noindent\textbf{Communication Complexity.} Each edge in the accumulation tree represents communication from a machine at a lower level to one at a higher level and contains four messages. 
They are the indices of the selected elements of size $k$, the size of the data associated with each selection (proportional to the size of each adjacency list ($ \leq \delta$), the total size of the data elements, and the data associated with each selection. 
Therefore the total volume of communication is $O(k\delta)$ per child. Since at each level, a parent node receives messages from $b$ children,
%communications from a node's children at each level, 
the communication complexity is $O(k\delta L b)$ for each parent. Therefore the communication complexity for the \randgreedi\ algorithm is $O(k\delta m)$ and for the \greedyl\ algorithm is $O(k\delta L \ceil{m^{1/L}}).$ 
We summarize these results in 
Table~\ref{tab:Complexity}.

\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|l|ccc}
    \toprule
        Algorithms & Metric & \greedy & \randgreedi & \greedyl \\
    \toprule
    \multirow{5}{15mm}{All}
        &Elements per leaf node & $n$ & $n/m $ & $n/m$ \\
        &Calls per leaf node & $nk$ & $nk/m $ & $nk/m$ \\
        &Elements per interior node & $0$ & $km$ & $k \ceil{m^{1/L}}$ \\
        &Calls per interior node & $0$ & $k^2m$ & $k^2 \ceil{m^{1/L}}$ \\
        &Total Function Calls & $kn$ & $k(n/m + km)$ & $k(n/m + Lk \ceil{m^{1/L}})$ \\ 
        \midrule 
        \multirow{4}{20mm}{$k$-cover / k-dominating set} 
        & & \multicolumn{3}{c}{$\delta$:subset size/number of neighbours} \\ 
        & Cost Per call & $\delta$ & $\delta$ & $\delta$ \\
        & Computational complexity & $\delta kn$ & $\delta k(n/m + km)$ & $\delta k(n/m + Lk \ceil{m^{1/L}})$\\
        & Communication cost & 0 & $\delta km$ & $\delta kL \ceil{m^{1/L}}$\\
        \midrule
        \multirow{5}{15mm}{$k$-medoid } 
        & & \multicolumn{3}{c}{$\delta$: number of features} \\
        & Cost Per call in Leaf node & $ \delta n$ & $\delta n/m $ & $\delta n/m $ \\ 
        &Cost Per call in interior node & 0 & $\delta km$ & $\delta k \ceil{m^{1/L}}$\\ 
        & Computational complexity & $\delta kn^2$ & $\delta k((n/m)^2 + (km)^2)$ & $\delta k((n/m)^2 + L(k \ceil{m^{1/L}})^2)$\\
        & Communication cost & 0 & $\delta km$ & $\delta kL \ceil{m^{1/L}}$ \\
        \bottomrule
    \end{tabular}}
    \caption{Complexity Results of the submodular functions for different algorithms. The number of elements in the ground set is $n$, the selection size is $k$, 
the number of machines is $m$, and the number of levels in the accumulation tree is $L$. }
    \label{tab:Complexity}
\end{table}

%in the Appendix. 
%Plot lb vs m
%Total complexity  



==> Latest/header.tex <==
\bibliographystyle{plainurl}


\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}


% Sets running headers as well as PDF title and authors
\title{A Parallel Algorithm for Maximizing Submodular Functions}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
%\title{An Example Article\thanks{Submitted to the editors DATE.
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

%\title{GreedyML: A Parallel Algorithm for Maximizing  Submodular Functions} %TODO Please add 

% Authors: full names plus addresses.


\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}



%\keywords{submodular optimization, approximation algorithm, parallel algorithm, data summarization} %TODO mandatory; please add comma-separated list of keywords

%\category{} %optional, e.g. invited paper

%\relatedversion{} %optional, e.g. full version hosted on arXiv, HAL, or other respository/website
%\relatedversiondetails[linktext={opt. text shown instead of the URL}, cite=DBLP:books/mk/GrayR93]{Classification (e.g. Full Version, Extended Version, Previous Version}{URL to related version} %linktext and cite are optional


==> Latest/omitted-tables.tex <==
%\section{Omitted Tables}
\label{app:omit-tab}
\begin{table}[htb]
    \centering
    \begin{tabular}{|c|c|c|} \hline
        Branching Factor & First accumulation & Final accumulation \\ \hline
        4  &0.74111	&0.99994 \\
        8  &0.82971	&1.00005 \\
        16 &0.91965	&0.99994 \\
        32 &1.00003	&1.00003 \\ \hline

    \end{tabular}
    \caption{Objective function values relative to the \greedy algorithm at the first and final accumulation steps for Friendster with selection size $k = 1000$ and $m = 32$.}
    \label{tab:quality-levels}
\end{table}

==> Latest/related-work.tex <==
\section{Related Work}
Barbosa et al.~\cite{barbosa}  have compared 
the \randgreedi\ algorithm with the sample and prune algorithm 
of Kumar et al.~\cite{Kumar}, and shown that the former performs better than the latter for practical quality of the computed approximate solution.  We observe this even though the second algorithm has a better worst-case approximation ratio in expectation. (The sample and prune algorithm  achieves an expected approximation of $1/(2+\epsilon)$ for $k$-cardinality  constraints, using $O(1/\delta)$ rounds,  when the memory per machine is $O(kn^\delta \: \log{n})$, where  $\delta > 0$ is a parameter, and $n$ is the number of elements in the ground set.) 

More recent work on distributed submodular maximization uses the multi-linear extension to map the problem into a continuous domain.  The authors of these papers  perform a gradient ascent on each local machine and build a consensus solution in each round, and  
%Mokhtari et al.\cite{Mokhtari}, and Alexander et al.\cite{Alexander} 
improve the approximation factor to $(1- 1/\mathrm e)$
~\cite{Chandra, Mokhtari, Alexander}.%\smf{What is $\epsilon$?. You mean ``e'' SG: Fixed}

However, we believe these latter papers represent primarily a theoretical contribution rather than one that leads to practical algorithms.
The reason is the high (exponential) cost of computing a single gradient by sampling many points; even randomized approximations of gradient computations are expensive.   
Most of these algorithms are not implemented and ones with implementation solve problems with hundred elements in the data set~\cite{Alexander}.
 

One potential criticism of our parallel algorithm is that the 
\emph{worst-case approximation ratios} achieved by it are lower, 
$\frac{1}{L} (1- 1/\mathrm e)$,  than the \randgreedi\ algorithm
($\frac{1}{2} (1- 1/\mathrm e)$),  when the number of levels $L>2$. 
However, 
our results show that the approximation ratios achieved in practice on several test problems do not show this loss in approximation quality with levels. 
This observation agrees  with the one of Barbosa et al. mentioned earlier in this section, 
and previous results on many matching and edge cover problems (e.g., see the surveys by Hougardy~\cite{Hougardy:survey} and 
Pothen, Ferdous and Manne~\cite{Pothen:Acta}). %. and Hougardy~\cite{Hougardy:survey}). 
 The latter article concludes that simpler algorithms with 
$1/2$- or $2/3-\epsilon$-approximation ratios for edge-weighted matching,  or $1/2$- or $2/3$-approximation ratios for vertex-weighted matching, achieve better practical approximation quality than a 
more involved $(1 -\epsilon)$-approximation algorithm. The former algorithms 
have more parallelism, are conceptually simpler, easier to implement,  and are practically 
orders of magnitude faster. 

